Instant Reality: Gaze-Contingent Perceptual Optimization for 3D Virtual Reality Streaming

Media streaming has been adopted for a variety of applications such as entertainment, visualization, and design. Unlike video/audio streaming where the content is usually consumed sequentially, 3D applications such as gaming require streaming 3D assets to facilitate client-side interactions such as object manipulation and viewpoint movement. Compared to audio and video streaming, 3D streaming often requires larger data sizes and yet lower latency to ensure sufficient rendering quality, resolution, and latency for perceptual comfort. Thus, streaming 3D assets can be even more challenging than streaming audios/videos, and existing solutions often suffer from long loading time or limited quality. To address this critical and timely issue, we propose a perceptually-optimized progressive 3D streaming method for spatial quality and temporal consistency in immersive interactions. Based on the human visual mechanisms in the frequency domain, our model selects and schedules the streaming dataset for optimal spatial-temporal quality. We also train a neural network for our model to accelerate this decision process for real-time client-server applications. We evaluate our method via subjective studies and objective analysis under varying network conditions (from 3G to 5G) and client devices (HMD and traditional displays), and demonstrate better visual quality and temporal consistency than alternative solutions.

==> dynamic_model.tex <==
\subsection{Visual Sensitivity to Dynamic Changes}
\input{popping}

\paragraph{Adaptive importance}
The sign of $\poppingIntensity$ is different in saccade and non-saccade cases.
We have:
\begin{align}
\label{eqn:adaptive}
\adaptive = \begin{cases}
-\poppingIntensity & \text{for non-saccade case}\\
\poppingIntensity & \text{for saccade case}\\
\end{cases}
\end{align}
This is because, for non-saccade case, we want to minimize the perceived popping effect.
And for saccade case, because of the saccade suppression, the popping effect is unlikely to be perceived, so we can transfer those with popping effect to avoid streaming them during non-saccade period and cause popping effect.

